The Boundary Condition for Some Isomonodromy Equations

In this article, we study a special class of Jimbo-Miwa-Mori-Sato isomonodromy equations, which can be seen as a higher-dimensional generalization of Painlev\'e VI. We first construct its convergent $n\times n$ matrix series solutions satisfying certain boundary condition. We then use the Riemann-Hilbert approach to prove that the resulting solutions are almost all the solutions. Along the way, we find a shrinking phenomenon of the eigenvalues of the submatrices of the generic matrix solutions in the long time behaviour.

==> Sect_GeneralSol.tex <==
\section{Almost every solution is a Shrinking solution}
\label{Sect:GeneralSol}

In this section, 
we will start with the monodromy data
% defined in Definition \ref{Def:MonoData}
\begin{align}
\label{Def:MD}
\tmop{MD}_{u,d} ( \Phi_n ) & \assign
(\nu_{u,d}(\Phi_n(z)),
\sigma(\Phi_n(z)),
\delta\Phi_n(z)),
\end{align} 
of the linear differential system \eqref{introisoStokeseq11},
which is also the first integral of 
the isomonodromy equation \eqref{zisoeq}
according to Proposition \ref{Pro:TrivalFirst}.
Note that in \eqref{Def:MD}, 
we need to require that $u$ belongs to
the universal covering $\Tilde{\Delta}$, 
rather than $\Delta=
\{u\in \mathbb{C}^n ~|~
u_i = u_j, \exists i,j \}$, 
in order to determine the value of $\Phi_n(z)$.

In Section \ref{subSect:ECfromMD},
we will base on 
the explicit Riemann-Hilbert mapping \eqref{Cat},
to provide a criterion 
by imposing some generic conditions on these monodromy data, 
to determine whether $\Phi_n(z)$ is a general solution.
In Section \ref{subSect:GP}, 
we will prove that those monodromy data
already form an open dense subset,
thus the set of general solutions $\Phi(z;\Phi_0)$,
associated to all boundary values $\Phi_0$ 
that satisfy the boundary condition, 
contains almost all solutions. 
% \input{Thm/Pro_isoM}
For convenience, let us introduce the following notations
\begin{nota}
\label{Nota:Mat}
For $n\times n$ matrix $\Phi=(a_{ij})_{n\times n}$,
\begin{itemize}
    \item denote $\Phi^{[k]}$ as the upper left $k\times k$
    submatrix, with eigenvalues
    $\lambda^{(k)}_1,\ldots,\lambda^{(k)}_k$;
    \item denote $\Phi^{[k]}_{\hat{k}k}$ as 
    the $k$-th column of $\Phi^{[k]}$
    but delete the $k$-th row;
    \item denote $\Phi^{[k]}_{k\hat{k}}$ as 
    the $k$-th row of $\Phi^{[k]}$
    but delete the $k$-th column.
\end{itemize}
For example, we have $\Phi^{[k]}=
\begin{pmatrix}
\Phi^{[k-1]} & \Phi^{[k]}_{\hat{k}k} \\
\Phi^{[k]}_{k\hat{k}} &  a_{kk}
\end{pmatrix}$.
\end{nota}

\begin{thm}
\label{Thm:GenisGen}
Suppose that $\Phi_n=(a_{i j})_{n\times n}$ 
is a solution of 
the $n$-th isomonodromy equation \eqref{zisoeq},
satisfy the following generic conditions
\begin{itemize}

\item $\Phi_n$ is non-resonant;

\item Take $V=\mathe^{2\pi\mathi M_d(u)}$, where
\begin{eqnarray}
\label{Cond:uPos}
\tmop{Im}(u_1\mathe^{\mathi d})
    >\cdots>
\tmop{Im}(u_n\mathe^{\mathi d}).
\end{eqnarray}
For every $1\leqslant k \leqslant n-1$,
there is a sequence
$\sigma_k=(\lambda^{(k)}_j)_{j=1,\ldots,k}$
satisfy that
\begin{align*}
\mathe^{2\pi\mathi \sigma_k}
=
\sigma(V^{[k]}),\quad
\sum_{j=1}^k \lambda^{(k)}_j
=
\sum_{j=1}^k a_{j j},\quad
|\tmop{Re}(\lambda^{(k)}_{j_1}-\lambda^{(k)}_{j_2})|
< 1, \quad
\text{for every $j_1,j_2$};
\end{align*}

\item Denote $\sigma(\Phi_n)=
(\lambda^{(n)}_j)_{j=1,\ldots,n}$,
for every $1\leqslant k \leqslant n-1$ we have
\begin{align*}
\lambda^{(k+1)}_{j_1}-\lambda^{(k)}_{j_2} \notin \mathbb{Z},
\quad
\text{for every $j_1,j_2$},
\end{align*}
\end{itemize}
then $\Phi_n$ is a general solution.
\end{thm}

\begin{prf}
The proof can be completed by combining 
Proposition \ref{Pro:nrGenCri} and 
Lemma \ref{Pro:SolveP0}. 
Note that
Proposition \ref{Pro:GenSGenc} ensures that 
these conditions are generic.
\end{prf}\\
\noindent
It can be seen that, 
for any $u$ and anti-Stokes direction $d$,
we can always make
a suitable index permutation 
such the condition
\eqref{Cond:uPos} hold.

\subsection{Effective Criterion from
Monodromy Data}
\label{subSect:ECfromMD}

In this section, 
from the monodromy data $\tmop{MD}_{u,d}(\Phi_n)$ of 
the solution $\Phi_n$,
we will use the explicit Riemann-Hilbert mapping \eqref{Cat}
provided by Theorem \ref{Thm:Cat}, 
to determine whether a solution $\Phi_n$
that satisfies the non-resonant condition is a general solution.
In Section \ref{subSect:NGS}, 
we will see that this criterion will fail 
under the resonant condition.
% Since it can be shown that 
% the monodromy data mapping $\tmop{MD}_{u,d}$ 
% is an injection on 
% the non-resonant matrix space $\mathfrak{gl}_n^{\tmop{nr}}$,
% as long as the monodromy data $\tmop{MD}_{u,d}(\Phi_n)$ 
% can be given by an $n\times n$ 
% constant matrix $\Phi_0\in\mathfrak{c}_0$
% through the explicit Riemann-Hilbert mapping \eqref{Cat}, 
% then $\Phi_n(z)$ must be 
% a general solution with $\Phi_0$ as the boundary value.
% Theorem \ref{Thm:AppCat} will introduces
% the more general form of 
% the explicit Riemann-Hilbert mapping \eqref{Cat},
% which covers the cases we are concerned with.
% For this, we need to introduce the following notations:
\begin{defi}
\label{Def:vcat}
For $n\times n$ matrix $\Phi_0$,
when $\Phi_0^{[2]},\ldots,\Phi_0^{[n-1]}$ is non-resonant,
we denote
\begin{align*}
\nu_{\tmop{cat}(\theta),d}(\Phi_0)
& \assign
\tmop{Ad}\left(
\overrightarrow{\prod^n_{k=1}}
C_{d+\theta_k}(E_k,\delta_k\Phi_0)
\right)
\mathe^{2\pi\mathi \Phi_0},\\
\tmop{MD}_{ \tmop{cat}(\theta),d } (\Phi_0)
& \assign
(\nu_{\tmop{cat}(\theta),d}(\Phi_0),
\sigma(\Phi_0),
\delta\Phi_0),\\
\mathscr{G}_{ + }
& \assign
\{ \tmop{MD}_{ \tmop{cat}(0), -\frac{\pi}{2} } (\Phi_0)
~|~ \Phi_0\in \mathfrak{c}_0 \}.
\end{align*}
% and we denote $\nu_{\tmop{cat},d}\assign
% \nu_{\tmop{cat}(0),d}$,
% $\mathscr{G}_{d} \assign \mathscr{G}_{\theta,d}$
% for short.
\end{defi}

\begin{lem}
\label{Lem:CoeftoMonoInj}
The monodromy data mapping
$\tmop{MD}_{u,d}$ 
defined in \eqref{Def:MD}
is an injection on
\begin{align*}
\mathfrak{gl}_n^{\tmop{nr}} \assign
\{\Phi \in \mathfrak{gl}_n ~|~
\Phi \text{ is non-resonant}\}.
\end{align*}
\end{lem}
\begin{prf}
Let us take
\begin{align*}
F_{d}(\xi;u,A)  = 
H_{d}(\xi;u,A) \xi^{\delta A}\mathe^{u \xi},\quad
F^{[\tmop{reg}]}(\xi;u,A)  =
H^{[\tmop{reg}]}(\xi;u,A) \xi^A,
\end{align*}
as the canonical fundamental solution of 
the confluent hypergeometric system
\begin{align*}
\frac{\mathd}{\mathd \xi} F(\xi) =
(u+A \xi^{-1})\cdot F(\xi),
\end{align*}
at $\xi = \infty$ and $\xi=0$, respectively.
Suppose that 
\[(\nu_{u,d}(A_1), \sigma(A_1), \delta A_1)
= (\nu_{u,d}(A_2), \sigma(A_2), \delta A_2),\]
from Lemma \ref{Lem:MtoExpM} we have
$M_d(u,A_1)=M_d(u,A_2)$,
and we denote as $M_d$.
According to \eqref{Md=ConjPhi} in
Proposition \ref{AppPro:FormSC} we have
\begin{align*}
F_{d}(\xi;u,A_1) F_{d}(\xi;u,A_2)^{-1} & =
H_{d}(\xi;u,A_1) H_{d}(\xi;u,A_2)^{-1}\\
& =
(H^{[\tmop{reg}]}(\xi;u,A_1) \Omega_d(u,A_1)^{-1}
\xi^{M_d})
(H^{[\tmop{reg}]}(\xi;u,A_1) \Omega_d(u,A_2)^{-1}
\xi^{M_d})^{-1}\\
& =
H^{[\tmop{reg}]}(\xi;u,A_1) \Omega_d(u,A_1)^{-1}
\Omega_d(u,A_2) H^{[\tmop{reg}]}(\xi;u,A_1)^{-1},
\end{align*}
thus $F(\xi)\assign F_{d}(\xi;u,A_1) F_{d}(\xi;u,A_2)^{-1}$
is analytic on 
the entire Riemann sphere $\mathbb{C}\cup\{\infty\}$,
and we have
\begin{align*}
I = F(\infty) = F(0) = \Omega_d(u,A_1)^{-1}\Omega_d(u,A_2),
\end{align*}
therefore we finish the proof.
\end{prf}

Although the non-resonant condition
only allows us to consider a part of the general solution, 
but we can reduce the problem to 
a characterization of the set 
$\tmop{MD}_{u,d}(\mathfrak{c}_n)$.
Therefore we need the following lemma.

\begin{lem}
\label{Lem:catComp}
  Denote $c_0 = 1$, for $c = (c_1, \ldots, c_n) \in (\mathbb{C}\backslash \{ 0
  \})^n$ we have
  \begin{align*}
    \tmop{Ad} \left( \overrightarrow{\prod_{k = 1}^n} C_{d +
    \theta_k} (c_k E_k, \delta_k \Phi_0) \right) \mathe^{2 \pi \mathi \Phi_0}
    & = 
    \nu_{\tmop{cat} (\theta + \arg c), d} \left( \left(
    \overrightarrow{\prod_{k = 1}^n} \left( \frac{c_k}{c_{k - 1}}
    \right)^{\tmop{ad} \delta_{k - 1} \Phi_0} \right) \Phi_0 \right).
  \end{align*}
\end{lem}

\begin{prf}
It can be verified directly from 
Proposition \ref{AppPro:FormSC}.
\end{prf}

% \begin{lem}
%   Denote $c_0 = 1$, for $c = (c_1, \ldots, c_n) \in (\mathbb{C}\backslash \{ 0
%   \})^n$ we have
%   \begin{align*}
%     \tmop{Ad} \left( \overrightarrow{\prod_{k = 1}^n} C_{d +
%     \theta_k} (c_k E_k, \delta_k \Phi_0) \right) \mathe^{2 \pi \mathi \Phi_0}
%     & = 
%     \nu_{\tmop{cat} (\theta + \arg c), d} \left( \left(
%     \overrightarrow{\prod_{k = 1}^n} \left( \frac{c_k}{c_{k - 1}}
%     \right)^{\tmop{ad} \delta_{k - 1} \Phi_0} \right) \Phi_0 \right).
%   \end{align*}
% \end{lem}

\begin{pro}
\label{Pro:nrGenCri}
% For $m\in\mathbb{Z}$,
% fixed $d\in ( (2m\mp\frac{1}{2})\pi - \frac{\pi}{2},
% (2m\mp\frac{1}{2})\pi + \frac{\pi}{2} )$.
Suppose that $\Phi_n(z)$ is a 
non-resonant solution of 
the $n$-th isomonodromy equation \eqref{zisoeq}
and \begin{align*}
\tmop{Im}(u_1\mathe^{\mathi d})
    >\cdots>
\tmop{Im}(u_n\mathe^{\mathi d}).
\end{align*}
then $\Phi_n(z)$ is a general solution
if and only if $\tmop{MD}_{u,d}(\Phi_n)\in
\mathscr{G}_{+}$.
% where $u\in\Tilde{\Delta}$ can take an arbitrary branch,
% and $d\in ( (2m\mp\frac{1}{2})\pi - \frac{\pi}{2},
% (2m\mp\frac{1}{2})\pi + \frac{\pi}{2} )$ and
% $u\in\Tilde{\Delta}$. is determined by requiring
% \begin{align*}
% \arg(u_{k+1}-u_{k})=0,
% \quad
% \text{for every $1\leqslant k \leqslant n-1$}.
% \end{align*}
\end{pro}

\begin{prf}
According to Lemma \ref{Lem:catComp} and
Theorem \ref{Thm:Cat}, 
we can assume that $d=-\frac{\pi}{2}$ and
\begin{align*}
\arg(u_k - u_{k-1} ) = 0,\quad
\text{for every }2\leqslant k \leqslant n,
\end{align*}
without loss of generality.
% From Proposition \ref{AppPro:FormSC},
% we can verify that
% \begin{align}
% \label{vcat2pi}
% \nu_{\tmop{cat}, d  }(\Phi_0) =
% \nu_{\tmop{cat}, d - 2m\pi}(
% \mathe^{- 2 m \pi \mathi \ad \delta \Phi_0}
% \Phi_0) =
% \nu_{\tmop{cat}, \mp\frac{\pi}{2} }(
% \mathe^{- 2 m \pi \mathi \ad \delta \Phi_0}
% \Phi_0)
% \end{align}
Therefore when $\Phi_0\in\mathfrak{c}_0$ we have
\begin{align*}
\tmop{MD}_{u,d}
(\mathcal{s}_n\cdots\mathcal{s}_1(\Phi_0)) =
\tmop{MD}_{\tmop{cat}(0), -\frac{\pi}{2} }(\Phi_0)
\in \mathscr{G}_{+} .
\end{align*}
Conversely, if there is a $\Phi_0\in\mathfrak{c}_0$ 
such that 
\begin{align*}
\tmop{MD}_{u,d} (\Phi_n)=
\tmop{MD}_{\tmop{cat}(0), -\frac{\pi}{2} }(\Phi_0) =
\tmop{MD}_{u,d} (\mathcal{s}_n\cdots\mathcal{s}_1(\Phi_0)),
\end{align*}
according to Lemma \ref{Lem:CoeftoMonoInj}, 
we have $\Phi_n =
\mathcal{s}_n\cdots\mathcal{s}_1(\Phi_0)$,
and we finish the proof.
\end{prf}

% \begin{defi}
%   \label{Def:trip}For $(C, \sigma_n, \Lambda) \in \mathscr{G}_{\theta, d}$,
%   define
%   \begin{eqnarray}
%     \overline{(C, \sigma_n, \Lambda)}^{- 1} & \assign & (\overline{C}^{- 1},
%     \overline{\sigma}_n, \overline{\Lambda}), \\
%     (C, \sigma_n, \Lambda)^{- \top} & \assign & (C^{- \top}, - \sigma_n, -
%     \Lambda), \\
%     (C, \sigma_n, \Lambda)^{\dagger} & \assign & (C^{\dagger}, -
%     \overline{\sigma}_n, - \overline{\Lambda}) . 
%   \end{eqnarray}
% \end{defi}
% \begin{cor}
% For $m \in \mathbb{Z}$ we have
% $\mathscr{G}_{ d + 2 m \pi} 
%  = \mathscr{G}_{d}$.
% \end{cor}
% \noindent
% Therefore, 
% $\mathscr{G}_{d}$ will actually only give two sets, 
% which is $\mathscr{G}_{+}$ and 
% $\mathscr{G}_{\frac{\pi}{2}}$.

\subsection{Inverse Monodromy Problems}
\label{subSect:GP}

% According to Proposition \ref{AppPro:StoTri},
% the Stokes matrices $S^+_{d}, S^-_{d}$
% are respectively an
% upper triangular matrix and a
% lower triangular matrix
% when we take $d=-\frac{\pi}{2}$, 
% thus the structure of 
% $\mathscr{G}_{+}$
% has the most natural structure.
% Therefore, 
% we need to study the structure of 
% $\mathscr{G}_{+}$ first, 
% and then base on this structure
% prove the generic property of the general solution.

This section will provide a sufficient condition 
for an element that belongs to $\mathscr{G}_{+}$. 
Although this only characterizes 
a proper subset of $\mathscr{G}_{+}$, 
it is still enough to allow us 
to prove the generic property of the general solution.
We will need to establish 
the inverse mapping of 
the Riemann-Hilbert mapping \eqref{Cat}
provided in Theorem \ref{Thm:Cat},
to produce $\Phi_0$.
Based on the results of Section \ref{step3}, 
we also can construct the pair $(u,\Phi_n(u))$ from $\Phi_0$, 
which is equivalent to solving the inverse monodromy problem.

\begin{lem}
\label{Pro:SolveP0}
If there exists
\begin{align*}
V \in  
\tmop{GL}_n(\mathbb{C}),\quad
\sigma_k = 
(\lambda^{(k)}_j)_{j=1,\ldots,k},\quad
\Lambda = 
\tmop{diag}(a_{11},\ldots,a_{nn}),
\end{align*}
for $1\leqslant k\leqslant n$,
such that
\begin{itemize}
    \item For $1\leqslant k\leqslant n-1$,
    \begin{subequations}
    \begin{eqnarray}
    \label{Cond:NonResk}
    \lambda^{(k)}_{j_1}-\lambda^{(k)}_{j_2}
    & \notin
    \mathbb{Z}\setminus\{0\},
    \quad
    \text{for every $j_1,j_2$},\\
    \label{Cond:NonResNear}
    \lambda^{(k+1)}_{j_1}-\lambda^{(k)}_{j_2}
    & \notin
    \mathbb{Z}\setminus\{0\},
    \quad
    \text{for every $j_1,j_2$};
    \end{eqnarray}
    \end{subequations}

    \item For $1\leqslant k\leqslant n$,
    \begin{subequations}
    \begin{align}
    \label{sigk:Exp}
        \mathe^{2\pi\mathi \sigma_k}
         & =
        \sigma(V^{[k]}),\\
    \label{sigk:Sum}
        \sum_{j=1}^k \lambda^{(k)}_j
         & =
        \sum_{j=1}^k a_{j j},
    \end{align}
    \end{subequations}
\end{itemize}
then there is a unique
$\Phi\in\mathfrak{gl}_n(\mathbb{C})$
such that
\begin{subequations}
\begin{align}
\tmop{MD}_{\tmop{cat}(0), -\frac{\pi}{2} } (\Phi) 
& =
(V,\sigma_n,\Lambda)\in
\mathscr{G}_{+},\\
\label{Cond:sigPk}
\sigma(\Phi^{[k]}) 
& =
\sigma_k,\quad
\text{for every $1\leqslant k \leqslant n$}.
\end{align}
\end{subequations}
\end{lem}

\begin{prf}
  Denote $d = - \frac{\pi}{2}$. Suppose that we have recursively calculated
  $\Phi^{[k - 1]}$ such that it 
  satisfies condition \eqref{Cond:sigPk}, 
  and
  \begin{align}
  \label{Ck-1rec}
    V^{[k - 1]} = 
    \tmop{Ad} \left( \overrightarrow{\prod_{j = 1}^{k - 1}}
    C_d (E_j, \delta_j \Phi^{[k - 1]}) \right) \mathe^{2 \pi \mathi
    \Phi^{[k - 1]}}.
  \end{align}
  For simplicity, let us denote
  \begin{align*}
    c_{k - 1} =  
    \overrightarrow{\prod_{j = 1}^{k - 1}} C_d (E_j,
    \delta_j \Phi^{[k - 1]}), \quad
    M_{k - 1} =  
    \tmop{Ad} (c_{k - 1}) \Phi^{[k - 1]}.
  \end{align*}
  Without loss of generality,
  we additionally
  assume that $\Phi^{[k - 1]}$ 
  has distinct eigenvalues,
  with spectral decomposition of $M_{k - 1}$
  \begin{align*}
    M_{k - 1} = 
    P_1 \lambda^{(k - 1)}_1 + \cdots + P_{k - 1} \lambda^{(k
    - 1)}_{k - 1}, 
  \end{align*}
  therefore we naturally have
  \begin{align}
  \label{CPCeigen}
    V^{[k]}_{k \hat{k}} P_i 
    V^{[k]}_{\hat{k} k}  =  - \prod_{p \neq i}
    \prod_j \frac{\mathe^{2 \pi \mathi \lambda^{(k - 1)}_i} - \mathe^{2 \pi
    \mathi \lambda^{(k)}_j}}{\mathe^{2 \pi \mathi \lambda^{(k - 1)}_i} -
    \mathe^{2 \pi \mathi \lambda^{(k - 1)}_p}} .
  \end{align}
  Next we construct $\Phi^{[k]} =  
    \left(\begin{array}{cc}
      \Phi^{[k - 1]} & \Phi^{[k]}_{\hat{k} k}\\
      \Phi^{[k]}_{k \hat{k}} & a_{k k}
    \end{array}\right)$
  under condition \eqref{Cond:NonResNear},
  where
\begin{subequations}
  \begin{align}
  \label{Form:Vcol}
    \Phi^{[k]}_{\hat{k} k} & =  
    \left( \frac{1}{2 \pi \mathi} \prod_{p, j}
    \frac{(\Phi^{[k - 1]} - \lambda^{(k)}_j I) !}{(\Phi^{[k - 1]} -
    \lambda^{(k - 1)}_p I) !} \right) \mathe^{- 2 \pi \mathi \Phi^{[k - 1]}}
    c_{k - 1}^{- 1} \cdot V^{[k]}_{\hat{k} k}, \\
  \label{Form:Vrow}
    \Phi^{[k]}_{k \hat{k}} & =  
    V^{[k]}_{k \hat{k}} \cdot c_{k - 1} \mathe^{-
    \pi \mathi (\Phi^{[k - 1]} + a_{k k} I)} \left( \frac{1}{2 \pi \mathi}
    \prod_{p, j} \frac{(\lambda^{(k)}_j I - \Phi^{[k - 1]}) !}{(\lambda^{(k -
    1)}_p I - \Phi^{[k - 1]}) !} \right) . 
  \end{align}
\end{subequations}
  From reflection formula and \eqref{CPCeigen} we have
  \begin{align*}
    &\quad \Phi^{[k]}_{k \hat{k}} \frac{1}{z I - \Phi^{[k - 1]}}
    \Phi^{[k]}_{\hat{k} k} \nonumber\\
    & =  V^{[k]}_{\hat{k} k} \mathe^{\pi \mathi (- 3 M_{k - 1} - a_{k k} I)}
    \left( \left( \frac{1}{2 \pi \mathi} \right)^2 \prod_{p, j}
    \frac{(\lambda^{(k)}_j I - M_{k - 1}) ! (M_{k - 1} - \lambda^{(k)}_j I)
    !}{(\lambda^{(k - 1)}_p I - M_{k - 1}) ! (M_{k - 1} - \lambda^{(k - 1)}_p
    I) !} \right) \frac{1}{z I - M_{k - 1}} V^{[k]}_{\hat{k} k} \nonumber\\
    & =  V^{[k]}_{\hat{k} k} \left( \mathe^{- 2 \pi \mathi M_{k - 1}}
    \prod_{p, j} \frac{\mathe^{2 \pi \mathi M_{k - 1}} - \mathe^{2 \pi \mathi
    \lambda^{(k - 1)}_p} I}{\mathe^{2 \pi \mathi M_{k - 1}} - \mathe^{2 \pi
    \mathi \lambda^{(k)}_j} I} \cdot \frac{M_{k - 1} - \lambda^{(k)}_j I}{M_{k
    - 1} - \lambda^{(k - 1)}_p I} \right) \frac{1}{z I - M_{k - 1}}
    V^{[k]}_{\hat{k} k} \nonumber\\
    & =  \sum_{i = 1}^{k - 1} V^{[k]}_{k \hat{k}} P_i V^{[k]}_{\hat{k} k}
    \cdot \left( \prod_{p \neq i} \prod_j \frac{\mathe^{2 \pi \mathi
    \lambda^{(k - 1)}_i} - \mathe^{2 \pi \mathi \lambda^{(k -
    1)}_p}}{\mathe^{2 \pi \mathi \lambda^{(k - 1)}_i} - \mathe^{2 \pi \mathi
    \lambda^{(k)}_j}} \cdot \frac{\lambda^{(k - 1)}_i -
    \lambda^{(k)}_j}{\lambda^{(k - 1)}_i - \lambda^{(k - 1)}_p} \right)
    \frac{1}{z - \lambda^{(k - 1)}_i} \nonumber\\
    & =  - \sum_{i = 1}^{k - 1} \left( \prod_{p \neq i} \prod_j
    \frac{\lambda^{(k - 1)}_i - \lambda^{(k)}_j}{\lambda^{(k - 1)}_i -
    \lambda^{(k - 1)}_p} \right) \frac{1}{z - \lambda^{(k - 1)}_i}, 
  \end{align*}
  therefore
  \begin{align*}
    \frac{\det (z I - \Phi^{[k]})}{\det (z I - \Phi^{[k - 1]})} = (z - a_{k
    k}) - \Phi^{[k]}_{k \hat{k}} \frac{1}{z I - \Phi^{[k - 1]}}
    \Phi^{[k]}_{\hat{k} k} = \prod_{p, j} \frac{z - \lambda^{(k)}_j}{z -
    \lambda^{(k - 1)}_p},
  \end{align*}
  thus $\sigma (\Phi^{[k]}) = \sigma_k$. From \eqref{Ck-1rec} and Proposition \ref{Pro:S} we have
  \begin{align*}
    V^{[k]} & =  \tmop{Ad} \left( \left(\begin{array}{cc}
      c_{k - 1} & 0\\
      0 & 1
    \end{array}\right) \right) \left( S_d^- (E_k, \Phi^{[k]})^{- 1}
    \left(\begin{array}{cc}
      \mathe^{2 \pi \mathi \Phi^{[k - 1]}} & 0\\
      0 & \mathe^{2 \pi \mathi a_{k k}}
    \end{array}\right) S_d^+ (E_k, \Phi^{[k]}) \right) \nonumber\\
    & =  \tmop{Ad} \left( \overrightarrow{\prod_{j = 1}^{k - 1}}
    C_d (E_j, \delta_j \Phi^{[k]}) \right) \cdot \tmop{Ad}
    (C_d (E_k, \Phi^{[k]})) \mathe^{2 \pi \mathi \Phi^{[k]}}
    \nonumber\\
    & =  \tmop{Ad} \left( \overrightarrow{\prod_{j = 1}^k} C_d
    (E_j, \delta_j \Phi^{[k]}) \right) \mathe^{2 \pi \mathi \Phi^{[k]}} . 
  \end{align*}
  Since condition \eqref{Cond:NonResk}
  ensures uniqueness, we have completed the proof.
\end{prf}

\begin{lem}
\label{Lem:LogSq}
Given a complex sequence
$c=(c_i)_{i=1,\ldots,k}$
and a constant $s$ 
such that
\begin{align*}
\mathe^{2\pi\mathi s} = c_1\cdots c_k,
\end{align*}
then there is a sequence
$\sigma=(\lambda_j)_{j=1,\ldots,k}$
such that
$\mathe^{2\pi\mathi \sigma} = c$,
$\sum_{j=1}^k \lambda_j = s$
and
\begin{eqnarray}
\label{Cond:ConsBoundy}
|\tmop{Re}(\lambda_{j_1}-\lambda_{j_2})|
\leqslant 1, \quad
\text{for every $j_1,j_2$}.
\end{eqnarray}
If we additionally have
\begin{eqnarray}
\label{Cond:ConsLem}
|\tmop{Re}(\lambda_{j_1}-\lambda_{j_2})|
 <  1, \quad
\text{for every $j_1,j_2$},
\end{eqnarray}
then the sequence $\sigma$ satisfying 
condition \eqref{Cond:ConsBoundy} is unique.
\end{lem}

\begin{prf}
Inductively assume that 
we have constructed the sequence
$s_m=(\lambda_{j,m})_{j=1,\ldots,k}$ 
satisfy that
\begin{align}
\label{Recsm}
\mathe^{2\pi\mathi s_m} = c,
\quad
\sum_{j=1}^k \lambda_{j,m} = s,
\end{align}
Assume that
\begin{align*}
\tmop{Re} \lambda_{j_1,m}  = 
\underset{1\leqslant j\leqslant k}{\tmop{min}}
\tmop{Re} \lambda_{j,m},\quad
\tmop{Re} \lambda_{j_2,m}  = 
\underset{1\leqslant j\leqslant k}{\tmop{max}}
\tmop{Re} \lambda_{j,m},
\end{align*}
if we have $\tmop{Re}(
\lambda_{j_2,m}-
\lambda_{j_1,m}) >1$,
then we can construct the sequence 
$s_{m+1}=(\lambda_{j,m+1})_{j=1,\ldots,k}$ as
\begin{align*}
  \lambda_{j, m + 1} = \left\{
  \begin{array}{ll}
    \lambda_{j, m} & ; j \neq j_1, j_2\\
    \lambda_{j, m} + 1 & ; j = j_1\\
    \lambda_{j, m} - 1 & ; j = j_2
  \end{array}\right..
\end{align*}
Therefore
$s_{m+1}$ also satisfy \eqref{Recsm},
and we either have
\begin{align*}
\underset{1\leqslant j_1,j_2\leqslant k}{\tmop{max}}
\tmop{Re}(
\lambda_{j_2,m+1}-
\lambda_{j_1,m+1}) <
\underset{1\leqslant j_1,j_2\leqslant k}{\tmop{max}}
\tmop{Re}(
\lambda_{j_2,m}-
\lambda_{j_1,m}),
\end{align*}
or
\begin{align*}
  \# \left\{ j_1 : \tmop{Re} \lambda_{j_1, m + 1} = \underset{1 \leqslant j
  \leqslant k}{\min} \tmop{Re} \lambda_{j, m + 1} \right\} & < \# \left\{
  j_1 : \tmop{Re} \lambda_{j_1, m} = \underset{1 \leqslant j \leqslant
  k}{\min} \tmop{Re} \lambda_{j, m} \right\}, \\
  \# \left\{ j_1 : \tmop{Re} \lambda_{j_2, m + 1} = \underset{1 \leqslant j
  \leqslant k}{\max} \tmop{Re} \lambda_{j, m + 1} \right\} & < \# \left\{
  j_1 : \tmop{Re} \lambda_{j_2, m} = \underset{1 \leqslant j \leqslant
  k}{\max} \tmop{Re} \lambda_{j, m} \right\}.
\end{align*}
Therefore for a sufficiently large $M$, 
we eventually have $\underset{1\leqslant j_1,j_2\leqslant k}{\tmop{max}}
\tmop{Re}(
\lambda_{j_2,M}-
\lambda_{j_1,M}) \leqslant 1$,
thus we finish the proof.
\end{prf}

\begin{pro}
\label{Pro:GenSGenc}
The general solutions are generic.
\end{pro}

\begin{prf}
Denote $\mathscr{G}_{+}^{\tmop{cl}}$
as the set of triples
$(V,\sigma_n,\Lambda)$
that satisfy the following conditions,
\begin{enumerate}
    \item $\sigma_n$ is a complex sequence 
    $(\lambda_j^{(n)})_{j=1,\ldots,n}$,
    such that
    $\mathe^{2\pi\mathi \sigma_n}$
    is the eigenvalues of $V$;
    
    \item $\Lambda$ is a diagonal matrix
    $\tmop{diag}(a_{11},\ldots,a_{nn})$, 
    such that
    $\mathe^{2\pi\mathi
    \sum_{j=1}^k a_{jj}}=
    \tmop{det}V^{[k]}$,
\end{enumerate}
which is exactly the closure of
$\mathscr{G}_{+}$,
and we introduce the following notation
\begin{align*}
\mathfrak{c}_0^{\mathrm{nr}}
& \assign 
\{\Phi_0\in\mathfrak{c}_0:
\text{$\Phi_0$ is non-resonant}
\},\\
\mathfrak{c}_n^{\mathrm{nr}}
& \assign 
\{\Phi_n(z)\in\mathfrak{c}_n:
\text{$\Phi_n(z)$ is non-resonant}
\},\\
\mathscr{G}_{+}^{\mathrm{nr}}
& \assign 
\{(V,\sigma_n,\Lambda)\in
\mathscr{G}_{+}:
(\sigma_n-\sigma_n)\cap
(\mathbb{Z}\setminus\{0\})
= \varnothing
\}.
\end{align*}
According to Proposition \ref{Pro:nrGenCri}, 
we have the following diagram.
\begin{eqnarray*}
\begin{tikzcd}
& \mathfrak{c}_n^{\mathrm{nr}} 
\arrow[dd, hook, "\cong"',
"{ \tmop{MD}_{u,d} }"] 
\arrow[rr, hook, "\subseteq"] &  & \text{non-resonant solutions} 
\arrow[dd, hook, 
"{ \tmop{MD}_{u,d} }"] \\
\mathfrak{c}_0^{\mathrm{nr}} 
\arrow[ru, "\cong"',
"\mathcal{s}_n\cdots\mathcal{s}_1"] 
\arrow[rd, "\cong",
"{\tmop{MD}_{\tmop{cat}(0),- \frac{\pi}{2}}}"']
&  &  & \\ &
\mathscr{G}_{+}^{\mathrm{nr}} 
\arrow[rr, hook, "\subseteq"]   &  &
\mathscr{G}_{+}^{\tmop{cl}}              
\end{tikzcd}
\end{eqnarray*}
According to Lemma \ref{Lem:LogSq}, 
for a generic elements 
$(V,\sigma_n,\Lambda)$
in $\mathscr{G}_{+}^{\tmop{cl}}$, 
we can derive a unique sequence 
$\sigma_k=(\lambda^{(k)}_j)_{j=1,\ldots,k}$
for $1\leqslant k\leqslant n-1$,
that satisfies
\begin{eqnarray}
|\tmop{Re}(
\lambda^{(k)}_{j_1}-
\lambda^{(k)}_{j_2})|
 <  1, \quad
\text{for every $j_1,j_2$},
\end{eqnarray}
under condition 
\eqref{sigk:Exp}, 
\eqref{sigk:Sum}.
At this time, 
condition \eqref{Cond:NonResk} 
is automatically satisfied, 
and generically there is also 
condition \eqref{Cond:NonResNear}, 
thus Lemma \ref{Pro:SolveP0} ensures that 
$\mathscr{G}_{+}^{\mathrm{nr}}$ 
is open dense in
$\mathscr{G}_{+}^{\tmop{cl}}$.
Finally, note that 
the space of non-resonant solutions is open dense, 
and the monodromy data mapping
$\tmop{MD}_{u,d}$ 
on this space is an analytic homeomorphism
to its image, 
thus the solution space $\mathfrak{c}_n^{\mathrm{nr}}$
is also open dense, 
and we complete the proof.
\end{prf}

==> Sect_RHatBound.tex <==
\section{Explicit Riemann-Hilbert Mapping}
\label{Sect:Cat}

Suppose that $\Phi(u)$ is a solution of
the $n$-th isomonodromy equation \eqref{isoeq}.
For fixed 
$u\in\mathbb{C}^n\setminus\Delta$,
let us consider the following $n\times n$ 
linear differential system
\begin{align}
\label{introisoStokeseq11}
\frac{\mathd}{\mathd \xi} F(\xi,u)
&=
\left(u+
\frac{\Phi(u)}{\xi}\right)\cdot F(\xi,u),
\end{align}
where we take
$u=\diag(u_1,\ldots,u_n)$
when $u$ represent a matrix.
The linear differential system
\eqref{introisoStokeseq11} 
has a canonical fundamental solution $F_d(\xi,u)$
at $\xi = \infty$,
and satisfy the following 
linear differential systems
with respect to $u_1,\ldots,u_n$,
\begin{equation}
\label{FxiuSys}
\left\{
\begin{alignedat}{3}
% R & L   &  R & L   &  R & L 
\frac{\partial}{\partial \xi}
F(\xi,u) 
& =
\left(u+
\frac{\Phi(u)}{\xi}
\right)\cdot F(\xi,u)\\
\frac{\partial}{\partial u_k}
F(\xi,u) 
& =
\left(E_k \xi+
\ad_u^{-1}\ad_{E_k}\Phi(u)
\right)\cdot F(\xi,u)
\end{alignedat}
\right..
\end{equation}
Therefore the isomonodromy equation
locally preserve the monodromy factor $\nu_{u,d}(\Phi(u))$
of the canonical fundamental solution $F_d(\xi,u)$,
which is
\begin{align*}
\nu_{u,d}(\Phi(u))\assign
F_d(\xi,u)^{-1}
F_d(\xi\mathe^{2\pi\mathi},u)
\end{align*}
and this is the origin of the term ‘isomonodromy’.
It should be emphasized that
$\nu_{u,d}(\Phi(u))$ is also depends on 
the argument of $u_1,\ldots,u_n$.
In particular, 
when $u_k$ is varied to 
$u_k\mathe^{2\pi\mathi}$, 
even though the position of $u$ remain unchanged, 
but the solution $\Phi(u)$ could be no longer the same,
thus $\nu_{u,d}(\Phi(u))$ could be different.

In section \ref{subSect:BasicODE}, 
we will introduce more details and concepts
on the canonical fundamental solution, 
the monodromy factor $\nu_{u,d}(\Phi)$,
the Stokes matrices $S_d^\pm(u,\Phi)$ and
the central connection matrices $C_d(u,\Phi)$
defined in Definition \ref{Def:MonoData}.
In section \ref{subSect:Fac},
we will start from the boundary value $\Phi_0$ of 
the general solution $\Phi(u;\Phi_0)$, 
to provide an explicit expression of 
the monodromy factor $\nu_{u,d}(\Phi(u;\Phi_0))$,
which is the explicit Riemann-Hilbert mapping at 
the caterpillar point $z_1,\ldots,z_n\to\infty$
for the general solution:

\begin{thm}[Caterpillar Formula]
\label{Thm:Cat}
Suppose that $\Phi(u;\Phi_0)$ is 
the general solution of 
the $n$-th isomonodromy equation \eqref{isoeq},
and the pair $(u,d)$ satisfy that
for every $1\leqslant k \leqslant n$
\begin{align}
\tmop{Im}(u_k \mathe^{\mathi d}) <
\min_{1\leqslant j < k} \tmop{Im}(u_j \mathe^{\mathi d}),
\quad \text{or }
\tmop{Im}(u_k \mathe^{\mathi d}) >
\max_{1\leqslant j < k} \tmop{Im}(u_j \mathe^{\mathi d}),
\end{align}
then we have
\begin{align}
\label{Cat}
\nu_{u,d}(\Phi(u;\Phi_0)) & =
\tmop{Ad}\left(
\overrightarrow{\prod^n_{k=1}}
C_{d+\arg(u_k- u_{k-1} )}(E_k,\delta_k\Phi_0)
\right)
\mathe^{2\pi\mathi
\Phi_0}.
\end{align}
\end{thm}
\begin{prf}
By applying Lemma \ref{Lem:CatPsi}.
\end{prf}

\begin{rmk}
Note that $\Phi_n(u)$ always need to restricted on
the covering space of
\begin{align*}
\{z\in\mathbb{C}^n ~|~
|z_k|>2,k=3,\ldots,n\}
\cong
\{u\in\mathbb{C}^n ~|~
u_k\notin\tmop{conv}\{u_1,\cdots,u_{k-1}\}
,k=2,\ldots,n\},
\end{align*}
Therefore, it is enough to determine 
the value of $\Phi_n(u)$ from 
the arguments $\arg(u_k-u_{k-1})$.
We will give the explicit expression of 
the central connection matrix $C_{d}(E_k,\delta_k\Phi_0)$
in Appendix \ref{App:Stokes}.
Finally, 
we will apply this explicit formula \eqref{Cat}
to prove that almost every solution is a general solution
in section \ref{Sect:GeneralSol}.
\end{rmk}
% Note that the general solution 
% $\Phi(u;\Phi_0)$ we defined 
% is a multivalued function with respect to 
% $z_k=\frac{u_k-u_{k-1}}{u_{k-1}-u_{k-2}}$, 
% therefore it is important 
% to specify the argument $\arg z_k$ 
% in order to clarify the meaning of $\Phi(z;\Phi_0)$.
% After taking the branch of $u_k$,
% we can determine the argument of $z_k$
% for $k=2,\cdots,n$ by noticing
% \begin{align*}
% \arg z_k =
% \arg(u_k-u_{k-1})-
% \arg(u_{k-1}-u_{k-2}),
% \end{align*}
% which can be used to
% recover $\Phi_0$ from $\Phi_n(z)$,
% and this explained the 
% right-hand side of \eqref{Cat}.
% Sometimes the set
% \begin{align*}
% -\bigcup_{k=2}^n 
% \left(
% \arg(u_k-\tmop{conv}\{u_1,\cdots,u_{k-1}\})
% +\mathbb{Z}\pi
% \right)
% \end{align*}
% could take the whole $\mathbb{R}$,
% unless we choose $z_3,\cdots,z_n$ big enough.
% At this time, 
% it will shrink to the set of
% anti-Stokes directions
% $-\bigcup_{k=2}^n 
% \left(
% \arg(u_k-u_{k-1})
% +\mathbb{Z}\pi
% \right)$, and
% $\arg z_k = \theta_k - \theta_{k-1}$.

\subsection{Confluent Hypergeometric Systems}
\label{subSect:BasicODE}

This subsection will organize 
the basic notations and properties 
of the confluent hypergeometric that people already know.
Most of the results and their proofs can be found in 
\cite{Balser}.


The \textbf{confluent hypergeometric system} 
is called an equation of the following form
\begin{eqnarray}
\label{Conflu}
\frac{\mathd}{\mathd \xi} F(\xi) =
\left(u+\frac{\Phi}{\xi}
\right)\cdot F(\xi),
\end{eqnarray}
where $\Phi$ is an $n\times n$ constant matrix,
the solution $F(\xi)$ is 
an $n\times n$ matrix-valued analytic function, and
\begin{itemize}
    \item $u=\diag(u_1 I_{n_1},\ldots, u_\nu I_{n_\nu})$,
    where $u_1,\ldots,u_\nu$ are distinct, 
    with multiplicity $n_1,\ldots,n_\nu$;
    \item system \eqref{Conflu} is divided into
    $(n_1,\ldots,n_\nu)$-blocks,
    and we denote $\Phi=(\Phi^{[i j]})_{\nu\times\nu}$
    as a block matrix.
\end{itemize}
The linear differential system \eqref{introisoStokeseq11}
associated with the isomonodromy equation \eqref{isoeq}
corresponds to the case of $n_1=\cdots=n_\nu=1$.
In order to introduce Theorem \ref{Thm:Cat}, 
we need to consider this general situation.

\begin{defi}
Let $\sigma(\Phi)$ denote the set of
eigenvalues of matrix $\Phi$, if
\begin{align*}
\left(
\sigma(\Phi)-\sigma(\Phi)
\right) \cap \mathbb{Z}
= \{0\},
\end{align*}
i.e. the difference between the eigenvalues of $\Phi$
does not take non-zero integers,
we called that $\Phi$ is \textbf{non-resonant}.
Otherwise, $\Phi$ is called \textbf{resonant}.
The set of $n\times n$ non-resonant matrix
is denoted as $\mathfrak{gl}_n^{\tmop{nr}}$.
\end{defi}

If $\Phi^{[11]},\ldots,\Phi^{[\nu\nu]}$
are non-resonant,
then the system \eqref{Conflu} has 
a unique formal fundamental solution of the following form
\begin{subequations}
\begin{align*}
F^{[\tmop{irr}]}(\xi) 
& =
H^{[\tmop{irr}]}(\xi)  \cdot 
\mathe^{u \xi} \xi^{
\delta_u \Phi
}\\
H^{[\tmop{irr}]}(\xi)
& =
I+\sum_{p=1}^{\infty} H_p^{[\tmop{irr}]} \xi^{-p},
\end{align*}
\end{subequations}
which is divergent in general,
and this is called the
\textbf{canonical formal fundamental solution of 
system \eqref{Conflu} at $\xi=\infty$},
where $\delta_u \Phi$ is called the 
\textbf{formal monodromy matrix},
\begin{align*}
\delta_u \Phi \assign
\diag(\Phi^{[11]},\ldots,\Phi^{[\nu\nu]}).
\end{align*}
If $\Phi$ is non-resonant,
then the system \eqref{Conflu} has 
a unique (formal) fundamental solution of the following form 
\begin{align*}
F^{[\tmop{reg}]}(\xi)
& =
H^{[\tmop{reg}]}(\xi) \cdot \xi^{\Phi}\\
H^{[\tmop{reg}]}(\xi) 
& =
I+\sum_{p=1}^{\infty} H_p^{[\tmop{reg}]} \xi^{p},
\end{align*}
which is convergent,
and this is called the
\textbf{canonical fundamental solution of 
system \eqref{Conflu} at $\xi=0$}. 

Although the canonical formal fundamental solution 
$F^{[\tmop{irr}]}(\xi)$
at $\xi=\infty$ is divergent, 
it is known that under Borel summation method, 
the formal solution $F^{[\tmop{irr}]}(\xi) $ can 
correspond to a family of analytic solutions 
$F_d(\xi)$. 
Let us introduce the notation of
the so-called \textbf{anti-Stokes direction},
which is defined 
as the direction on the logarithmic Riemann surface 
with the following real numbers as argument
\begin{align*}
\tmop{aS}(u)\assign
\{
{-\arg (u_i-u_j)
+2k\pi:k\in\mathbb{Z},i\neq j}
\},
\end{align*}
we arrange these argument into 
a strictly monotonically increasing sequence
\begin{align*}
\cdots< \tau_{-1} < \tau_{0} < \tau_1 < \cdots.
\end{align*} 
For $d\in(\tau_j,\tau_{j+1})$, 
the \textbf{Stokes sector} is denoted as
the sectorial regions
\begin{align*}
\tmop{Sect}_d\assign
\{\xi\in\tilde{\mathbb{C}}:
\arg \xi\in (\tau_j-\frac{\pi}{2},\tau_{j+1}+\frac{\pi}{2})
\},
\end{align*}
which contains the ray $\arg \xi = d$,
such that on each of these sectors 
there is a unique
analytic solution $F_d(\xi)$
with the prescribed asymptotics 
$F^{[\tmop{reg}]}(\xi)$,
called the
\textbf{canonical fundamental solution of 
system \eqref{Conflu} at $\xi=\infty$
with respect to direction $d$}.
These canonical fundamental solutions at $\xi=\infty$
are in general different 
(that reflects the Stokes phenomenon), 
and the transition between them 
can be measured by Stokes matrices 
$S_d^\pm(u,\Phi(u))$
defined in Definition \ref{Def:MonoData}.

The following lemma allows us to 
well-define the concept of 
the monodromy matrix 
of the canonical fundamental solution $F_d(\xi)$
in the non-resonant case.

\begin{lem}
\label{Lem:MtoExpM}
If $M$ is non-resonant, 
We have the following bijection
\begin{align*}
\mathfrak{gl}_n^{\tmop{nr}} & \rightarrow
\{(V,(\lambda_i)_{i=1,\ldots,n}) ~|~
\sigma(V) = (\mathe^{2\pi \mathi \lambda_i})_{i=1,\ldots,n},
\forall i,j.
\lambda_i - \lambda_j \notin 
\mathbb{Z}\setminus\{0\} \}\\
(\mathe^{2\pi \mathi (\cdot)},\sigma):
M & \mapsto
(\mathe^{2\pi \mathi M},
\sigma(M)).
\end{align*}
\end{lem}
% \begin{prf}
% Suppose that $\mathe^{2\pi \mathi M_1} = \mathe^{2\pi \mathi M_2}$
% and $\sigma(M_1) = \sigma(M_2)$, 
% take the Jordan normal form
% \begin{eqnarray}
% P \mathe^{2\pi \mathi M_1} P^{-1} =
% P \mathe^{2\pi \mathi M_2} P^{-1} =
% \diag (J_1,\ldots,J_\nu).
% \end{eqnarray}
% According to $\sigma(M_1) = \sigma(M_2)$,
% and the difference between eigenvalues is not a nonzero integer, 
% it follows that
% there exists a unique integers sequence 
% $n_1,\ldots,n_\nu$ such that
% \begin{eqnarray}
% P^{-1}\left(
% \frac{1}{2\pi\mathi} \ln
% \diag (J_1,\ldots,J_\nu) +
% \diag (n_1 I_1,\ldots,n_\nu I_\nu)
% \right)P = M_i,
% \end{eqnarray}
% thus $M_1=M_2$.
% \end{prf}

\begin{defi}
\label{Def:MonoData}
Suppose that 
$\Phi^{[11]},\ldots,\Phi^{[\nu\nu]}$
are non-resonant
\begin{itemize}

\item For every $d\notin \tmop{aS}(u)$,
we define the \textbf{Stokes matrices} as
\begin{align*}
S_d^{\pm}(u,\Phi) \assign 
F_{d\pm\pi}(\xi)^{-1} F_d(\xi),
\end{align*}
and we denote the \textbf{monodromy factor}
of $F_d(\xi)$ as
\begin{align*}
\nu_{u,d}(\Phi)\assign
F_d(\xi)^{-1} F_d(\xi\mathe^{2\pi\mathi});
\end{align*}
% sometimes we simply
% denote as $\nu_u(\Phi)$;
% We call the \textbf{monodromy data} as 
% the following triple
% \begin{align*}
% \tmop{MD}_{u,d} \assign
% (\nu_{u,d}(\Phi), \sigma(\Phi), \delta_u\Phi);
% \end{align*}

\item If we additionally suppose that 
$\Phi$ is non-resonant, then we
define the \textbf{central connection matrices} as
\begin{align*}
C_d(u,\Phi)\assign
F_d(\xi)^{-1} F^{[\tmop{reg}]}(\xi),
\end{align*}
and we define the 
\textbf{(canonical) monodromy matrix} $M_d(u)$
of the canonical fundamental solution $X_d(t)$
by requiring 
\begin{align*}
(\mathe^{2\pi\mathi M_d(u)},
\sigma(M_d(u)))
=
(\nu_{u,d}(\Phi),
\sigma(\Phi)).
\end{align*}
In general, as long as $\mathe^{2\pi\mathi M}$ is a monodromy factor, 
people will call $M$ monodromy matrix.
\end{itemize}
\end{defi}

\begin{pro}
\label{AppPro:FormSC}
If $\Phi^{[11]}, \ldots, \Phi^{[\nu \nu]}$ are non-resonant,
then we have
\begin{subequations}
\begin{align}
  \label{LUDecomp}
    \nu_{u, d} (\Phi) 
    & = 
    S^-_d (u, \Phi)^{- 1} \cdot \mathe^{2 \pi \mathi
    \delta_u \Phi} \cdot S^+_d (u, \Phi), \\
    S^{\pm}_{d + 2 k \pi} (u, \Phi) 
    & = 
    \mathe^{- 2 k \pi \mathi \delta_u
    \Phi} \cdot S^{\pm}_d (u, \Phi) \cdot \mathe^{2 k \pi \mathi \delta_u
    \Phi}, \quad k \in \mathbb{Z}, \\
    S^{\pm}_{d \mp \pi} (u, \Phi) 
    & = 
    S^{\mp}_d (u, \Phi)^{- 1},
\end{align}
\end{subequations}
and for $c\in\mathbb{C}\setminus\{0\}$ we have
\begin{subequations}
\begin{align}
S_d^\pm(c u, \Phi) & =
c^{\delta_u \Phi}
S_{d+\arg c}^\pm(u, \Phi)
c^{- \delta_u \Phi},\\
S_d^\pm(\overline{u}, \overline{\Phi})  =
\overline{S_{-d}^\mp(u, \Phi)},\quad
S_d^\pm(-u^\top, -\Phi^\top) & =
S_{d}^\pm(u, \Phi)^{-\top},\quad
S_d^\pm(-u^\dagger, -\Phi^\dagger)  =
S_{-d}^\mp(u, \Phi)^{-\dagger}.
\end{align}
\end{subequations}
If $\Phi$ and 
$\Phi^{[11]}, \ldots, \Phi^{[\nu \nu]}$ are non-resonant,
then we have
\begin{subequations}
\begin{align}
\label{Md=ConjPhi}
    M_d (u, \Phi) 
    & = 
    C_d (u, \Phi) \cdot \Phi \cdot C_d (u,
    \Phi)^{- 1}, \\
    C_{d + 2 k \pi} (u, \Phi) 
    & = 
    \mathe^{- 2 k \pi \mathi \delta_u
    \Phi} \cdot C_d (u, \Phi) \cdot \mathe^{2 k \pi \mathi \Phi}, \quad k
    \in \mathbb{Z}, \\
    C_{d \pm \pi} (u, \Phi) 
    & = 
    S^{\pm}_d (u, \Phi) \cdot C_d (u,
    \Phi),
\end{align}
\end{subequations}
and for $c\in\mathbb{C}\setminus\{0\}$ we have
\begin{subequations}
\begin{align}
\label{PropC:cu}
C_d(c u, \Phi) & =
c^{\delta_u \Phi}
C_{d+\arg c}(u, \Phi)
c^{- \Phi},\\
C_d(\overline{u}, \overline{\Phi})  =
\overline{C_{-d}(u, \Phi)},\quad
C_d(-u^\top, -\Phi^\top) & =
C_{d}(u, \Phi)^{-\top},\quad
C_d(-u^\dagger, -\Phi^\dagger)  =
C_{-d}(u, \Phi)^{-\dagger}.
\label{PropC:uT}
\end{align}
\end{subequations}
\end{pro}

\subsection{Factorization}
\label{subSect:Fac}

Suppose that 
$\Phi_n(z_n)\in \mathfrak{s}_{n}(\bm{z}_{n-1})$,
which means it is the solution of
the $n$-th isomonodromy equation \eqref{kzisoode}
with respect to $z_n$,
and satisfied
\begin{itemize}
    \item shrink phenomenon 
    \eqref{Cond:BoundEigenLim};

    \item control conditions
    \eqref{Cond:BounddkPk}, \eqref{Cond:BoundPk}.
\end{itemize}
From Proposition \ref{Lem:ControlisEnough},
there is a $n\times n$ matrix 
$\Phi_{n-1} \in \mathfrak{b}_{n-1}(\rm{pt})$
such that
\begin{subequations}
\begin{align}
\label{dPnrmvar}
\delta_{n-1}
\Phi_n(z_n) &=
\delta_{n-1}
\Phi_{n-1} +
O(z_n^{-\varepsilon}),
\quad z_n\to\infty,
\\
\label{Pnrmvar}
z_n^{\ad\delta_{n-1}
\Phi_{n-1}}
\Phi_n(z_n) &=
\Phi_{n-1} +
O(z_n^{-\varepsilon}),
\quad z_n\to\infty
\end{align}
\end{subequations}
Fixed $\bm{z}_{n-1} = (z_1,\ldots,z_{n-1})$, 
rewrite the
linear differential systems
\eqref{FxiuSys}
as follows
\begin{equation}
\label{Sysxizn}
\left\{
\begin{alignedat}{3}
% R & L   &  R & L   &  R & L 
\frac{\partial}{\partial \xi}
F(\xi,z_n) 
& =
\left(u+
\frac{\Phi_n(z_n)}{\xi}
\right)\cdot F(\xi,z_n) \\
\frac{\partial}{\partial z_n}
F(\xi,z_n) 
& =
\left(\frac{\partial u}{\partial z_n}\xi+
\ad_u^{-1}
\ad_{\partial u/\partial z_n}\Phi_n(z_n)
\right)\cdot F(\xi,z_n) 
\end{alignedat}
\right.,
\end{equation}
and consider 
the coordinate transformation:
$\left\{
\begin{alignedat}{3}
% R & L   &  R & L   &  R & L 
x     & = \xi\\
\zeta_n & = \xi z_n
\end{alignedat}
\right.$,
we can obtain 
the following linear differential systems
\begin{lem}
Denote
\begin{equation}
\label{xzetaSys}
\left\{
\begin{alignedat}{3}
% R & L   &  R & L   &  R & L 
\frac{\partial}{\partial x} 
F (x, \zeta_n)
& =
A_1(x,\zeta_n)
\cdot F (x, \zeta_n) \\
\frac{\partial}{\partial \zeta_n} 
\left(\left(
\frac{\zeta_n}{x}\right)^
{\delta_{n-1}\Phi_{n-1}}
F(x,\zeta_n)\right)
& =
A_2(x,\zeta_n)
\cdot 
\left(
\frac{\zeta_n}{x}\right)
^{\delta_{n - 1}\Phi_{n - 1}} 
F (x, \zeta_n)
\end{alignedat}
\right..
\end{equation}
When $x\to 0,\zeta_n\to\infty$, we have
\begin{align}
A_1(x,\zeta_n) &=
u^{(n)} +
\frac{\delta_{n - 1} \Phi_{n - 1}}{x} + 
O (x^{-1+\varepsilon} \zeta_n^{- \varepsilon})\\
A_2(x,\zeta_n) &=
\frac{\partial u_n}{\partial z_n} E_n +
\frac{\Phi_{n - 1}}{\zeta_n} + 
O (x^{\varepsilon} \zeta_n^{-1-\varepsilon}),
\end{align}
where $u^{(n)}=\diag(
u_1,\ldots,u_{n-1},u_{n-1}
)$.
\end{lem}


\begin{prf}
From \eqref{TkExp}, \eqref{z1zk-1Dkk:Expression}
and \eqref{Eq:dk-1pk}, we have
\begin{align*}
\tmop{ad}_u^{- 1} 
\tmop{ad}_{\partial u / \partial z_n} 
\Phi_n (z_n) & =
z_n^{- 1} \delta_{n - 1}^{\bot} 
\Phi_n (z_n) + 
z_n^{-2}
\ad_{U_{(n)}/(\Tilde{I}_{n-1}+z_n^{-1}U_{(n)})}
\ad_{E_n}\Phi_n(z_n),
\end{align*}
therefore
from \eqref{dPnrmvar}, \eqref{Pnrmvar}
\begin{align}
\nonumber
A_1(x,\zeta_n) &=
\frac{\partial \xi}{\partial x} 
\left( u + \frac{\Phi_n (z_n)}{\xi}
\right) + 
    \frac{\partial z_n}{\partial x} \left( \frac{\partial
    u}{\partial z_n} \xi + \tmop{ad}_u^{- 1} \tmop{ad}_{\partial u / \partial
    z_n} \Phi_n (z_n) \right)\\
\nonumber
& = 
u^{(n)} + 
\frac{\delta_{n-1}\Phi_n(z_n)}{x}- 
\frac{1}{\zeta_n}
\ad_{U_{(n)}/(\Tilde{I}_{n-1}+z_n^{-1}U_{(n)})}
\ad_{E_n}\Phi_n(z_n)\\
\label{A1expan}
& = u^{(n)} + \frac{\delta_{n - 1} \Phi_{n - 1}}{x} + 
    O (x^{-1+\varepsilon}
    \zeta_n^{- \varepsilon}), 
\quad 
x \rightarrow 0, 
\zeta_n \rightarrow \infty,
\end{align}
  and
\begin{align}
\nonumber
A_2(x,\zeta_n) 
&=
\left(
\frac{\zeta_n}{x}\right)^
{\ad\delta_{n-1}\Phi_{n-1}} 
\frac{\partial
    z_n}{\partial \zeta_n} \left( \frac{\partial u}{\partial z_n} \xi +
    \tmop{ad}_u^{- 1} \tmop{ad}_{\partial u / \partial z_n} \Phi_n (z_n)
    \right) + \frac{\delta_{n - 1} \Phi_{n - 1}}{\zeta_n}\\
\nonumber
& =  
\left(
\frac{\zeta_n}{x}\right)^
{\ad\delta_{n-1}\Phi_{n-1}}
\left(
    \frac{\partial u_n}{\partial z_n} E_n + \frac{1}{x} \tmop{ad}_u^{- 1}
    \tmop{ad}_{\partial u / \partial z_n} \Phi_n (z_n) \right) +
    \frac{\delta_{n - 1} \Phi_{n - 1}}{\zeta_n}\\
\label{A2expan}
& = 
\frac{\partial u_n}{\partial z_n} E_n + 
\frac{\Phi_{n -1}}{\zeta_n} + O (x^{\varepsilon} \zeta_n^{- 1 - \varepsilon}),
\quad 
x \rightarrow 0, 
\zeta_n \rightarrow \infty,
\end{align}
  thus we finish the proof.
\end{prf}

Let us introduce the following notation 
for some canonical fundamental solutions
\begin{itemize}
\item 
$F(\xi,z_n) =
H(\xi,z_n)
\xi^{\Phi_n(z_n)}$ as 
the canonical fundamental solution of 
system \eqref{Sysxizn}
for fixed $z_n$
at $\xi = 0$,
and
$F_d(\xi,z_n) =
H_d(\xi,z_n)
\xi^{\delta\Phi}
\mathe^{u \xi}$ as 
the canonical fundamental solution
for fixed $z_n$
at $\xi = \infty$ 
with respect to direction $d$;


\item 
$F^{[0]} (x, \zeta_n) =
H^{[0]} (x, \zeta_n)
x^{\delta_{n-1}\Phi_{n-1}}$ as 
the canonical fundamental solution of 
systems \eqref{xzetaSys} 
for fixed $\zeta_n$
at $x = 0$;

% \item $F^{[n]}_d (x, \zeta_n)=
% \left(\left(
% \frac{\zeta_n}{x}\right)^
% {-\ad\delta_{n-1}\Phi_{n-1}}
% H^{[n]}_d (x, \zeta_n)\right)
% x^{\delta_{n-1}\Phi_{n-1}}
% \mathe^{(u_{n-1}-u_{n-2})\zeta_n E_n}$ as 
% the canonical fundamental solution of
% system \eqref{xzetaSys} 
% at $\zeta_n = \infty$ with respect to 
% direction $d$.
  
\item $T^{[0]} (x)=
Y^{[0]} (x)
x^{\delta_{n-1}\Phi_{n-1}}$
as the canonical fundamental solution of 
the following system at $x = 0$
  \begin{align}
    \frac{\partial}{\partial x} T (x)  =  \left( u^{(n)} + \frac{\delta_{n -
    1} \Phi_{n - 1}}{x} \right) \cdot T (x),
  \end{align}
and 
$T^{[0]}_d(x)=Y^{[0]}_d(x)
x^{\delta\Phi}
\mathe^{u^{(n)}x}$ as 
the canonical fundamental solution 
at $x = \infty$ 
with respect to direction $d$;

\item $T^{[n]} (\zeta_n)=
Y^{[n]} (\zeta_n)
\zeta_n^{\Phi_{n-1}}$
as the canonical fundamental solution of 
the following system at $\zeta_n = 0$
  \begin{align}
  \label{Eq:T2}
    \frac{\partial}{\partial \zeta_n} T (\zeta_n)  =  \left( \frac{\partial
    u_n}{\partial z_n} E_n + \frac{\Phi_{n - 1}}{\zeta_n} \right) \cdot T
    (\zeta_n).
  \end{align}
and
$T^{[n]}_d (\zeta_n) =
Y^{[n]}_d (\zeta_n)
\zeta_n^{\delta_{n-1}\Phi_{n-1}}
\mathe^{(u_{n-1}-u_{n-2})\zeta_n E_n}$ as 
the canonical fundamental solution 
at $\zeta_n = \infty$ 
with respect to direction $d$
\end{itemize}

\begin{lem}
\label{Lem:CatPic}
The canonical fundamental solutions have the following locally uniform limits.
\begin{itemize}
\item Fixed $\zeta_n$,
when $x\to 0$ we locally uniformly have
\begin{align}
\label{Lim:adH1}
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}} 
H^{[0]}(x,\zeta_n) 
&\xrightarrow{x\to 0} I,\\
\label{Lim:addH1}
\frac{\partial }
{\partial \zeta_n}
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}} 
H^{[0]}(x,\zeta_n)
&\xrightarrow{x\to 0} 0,\\
\label{Lim:adH}
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}} 
H(x,\zeta_n/x)
&\xrightarrow{x\to 0}
Y^{[n]}(\zeta_n);
\end{align}

\item Fixed $x$,
when $\zeta_n\to\infty$ we locally uniformly have
\begin{align}
\label{Lim:H1}
H^{[0]}(x,\zeta_n)
&\xrightarrow{\zeta_n\to \infty}
Y^{[0]}(x);
\end{align}

\item Fixed $x$,
when $\zeta_n\to\infty$
with $\arg \zeta_n\in
(d_{\zeta_n}-\varepsilon,
 d_{\zeta_n}+\varepsilon)$,
we locally uniformly have
\begin{align}
\label{Lim:Hd}
H_{d_x}(x,\zeta_n/x)
&\xrightarrow{\zeta_n\to \infty}
Y_{d_x}^{[0]}(x),\\
\label{Lim:adYd}
\zeta_n^{-\ad
\delta_{n-1}\Phi_{n-1}}
Y_{d_{\zeta_n}}^{[n]}(x,\zeta_n)
&\xrightarrow{\zeta_n\to \infty}I,
\end{align}
where $d_x\assign \arg x$.
\end{itemize}
\end{lem}

\begin{prf}
For convenience,
we will only provide the proofs for 
\eqref{Lim:adH1}, \eqref{Lim:addH1}.
% , and \eqref{Lim:H1}
The approach for the rest
are similar, 
% but \eqref{Lim:Hd} and \eqref{Lim:adYd}
% need to 
% be transformed into convergent power series 
% by considering the Borel-Laplace transformation, 
see \cite{Xu} for more details.

Denote
$\Tilde{H}^{[0]}(x,\zeta_n)=
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}} 
H^{[0]}(x,\zeta_n)$.
Note that 
$\Tilde{H}^{[0]}(x,\zeta_n)$
% and $\Tilde{Y}^{[0]}(x)$
satisfy the following equation
% respectively
\begin{align*}
\frac{\partial}{\partial x} \Tilde{H}^{[0]}(x,\zeta_n) 
& = \left( 
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}}
A_1 (x,\zeta_n) -
\frac{\delta_{n-1}\Phi_{n-1}}{x}
\right) \cdot 
\Tilde{H}^{[0]}(x,\zeta_n),
    % \\
    % \frac{\partial}{\partial x} 
    % \Tilde{Y}^{[0]}(x)
    % & = \left( x^{- \tmop{ad}
    % \delta_{n - 1} \Phi_{n - 1}} 
    % u^{(n)} \right) \cdot 
    % \Tilde{Y}^{[0]}(x),
\end{align*}
For $|x|< h$
with bounded argument,
from \eqref{A1expan}
we can verify 
there exists a constant $C$ 
independent of $h$, 
such that
\begin{align*}
\left\| 
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}}
A_1 (x,\zeta_n) -
\frac{\delta_{n-1}\Phi_{n-1}}{x}
\right\| & \leqslant  
C \cdot 
|x|^{-1 +\varepsilon},\\
\left\|
\frac{\partial}
{\partial \zeta_n}
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}}
A_1 (x,\zeta_n)\right\| 
& \leqslant  
C \cdot 
|x|^{-1+\varepsilon},
\end{align*}
  Considering 
  the Picard iteration of 
  the corresponding equation
  with $P_0(x,\zeta_n)=I$
  \begin{align*}
    P_m (x, \zeta_n) & = 
    I + \int_0^x \left( 
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}}
A_1 (x,\zeta_n) -
\frac{\delta_{n-1}\Phi_{n-1}}{x}
    \right) \cdot P_{m - 1} (x, \zeta_n) \mathd x,\\
    \nonumber
    \frac{\partial P_m (x, \zeta_n)}{\partial \zeta_n} 
    & = \int_0^x \left(
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}}
A_1 (x,\zeta_n) -
\frac{\delta_{n-1}\Phi_{n-1}}{x}
    \right) \cdot \frac{\partial P_{m -
    1} (x, \zeta_n)}{\partial \zeta_n} \mathd x\\
    &\phantom{=}
    + \int_0^x \left( 
\frac{\partial}
{\partial \zeta_n}
\left(
\frac{\zeta_n}{x}
\right)^{\ad\delta_{n-1}\Phi_{n-1}}
A_1 (x,\zeta_n)
    \right) \cdot P_{m - 1}
    (x, \zeta_n) \mathd x,
  \end{align*}
and introduce the following norm
  \begin{align*}
    \| F \|_{\varepsilon,h} 
    & \assign 
    \underset{0 < x < h}{\sup} \| x^{-
    \varepsilon} F (x) \|,
  \end{align*}
  there exists a constant $C_0$ 
  independent of $h$, 
  such that
  \begin{align*}
\| P_{m+1}-P_m \|_{\varepsilon,h}
& \leqslant 
C_0 |h|^{\varepsilon} 
\cdot 
\| P_m-P_{m-1} \|_{\varepsilon,h},\\
\left\| 
\frac{\partial P_{m+1}}{\partial \zeta_n} - 
\frac{\partial P_{m  }}{\partial \zeta_n}
\right\|_{\varepsilon,h}
& \leqslant C_0 |h|^{\varepsilon} 
\cdot
\left(
\| P_{m  }-P_{m-1} \|_{\varepsilon,h}
+
\left\| 
\frac{\partial P_{m  }}{\partial \zeta_n} - 
\frac{\partial P_{m-1}}{\partial \zeta_n} 
\right\|_{\varepsilon,h}
\right).
\end{align*}
Therefore
$P_m$ and
$\frac{\partial P_{m  }}{\partial \zeta_n}$
are locally uniformly convergent to
$\Tilde{H}^{[0]}(x,\zeta_n)$ and 
$\frac{\partial \Tilde{H}^{[0]}(x,\zeta_n)}
{\partial \zeta_n}$, 
and we have
\begin{align*}
\Tilde{H}^{[0]}(x,\zeta_n)
& = I+O(x^\varepsilon),
\quad x\to 0,\\
\frac{\partial \Tilde{H}^{[0]}(x,\zeta_n)}
{\partial \zeta_n}
& = O(x^\varepsilon),
\quad x\to 0,
\end{align*}
thus we proved
\eqref{Lim:adH1} and \eqref{Lim:addH1}.
\end{prf}

\begin{lem}
\label{Lem:PreCat}
Suppose that
\begin{align}
\label{Cond:NonDengStokesS}
\tmop{Im}(u_n \mathe^{\mathi d_x}) <
\min_{1\leqslant k < n} \tmop{Im}(u_k \mathe^{\mathi d_x}),
\quad \text{or }
\tmop{Im}(u_n \mathe^{\mathi d_x}) >
\max_{1\leqslant k < n} \tmop{Im}(u_k \mathe^{\mathi d_x}),
\end{align}
we have
\begin{align}
\nonumber
F_{d_x}(x,\zeta_n/x) \cdot
C_{d_x} (u,\delta_{n-1}\Phi_{n-1})
&=
F^{[0]}(x,\zeta_n) \cdot 
\zeta_n^{-\delta_{n-1} \Phi_{n-1}}
T^{[n]}_{d_{\zeta_n}} (\zeta_n)\\
\label{PreCat}
&=
F_{d_{\zeta_n}}^{[n]}(x,\zeta_n) \cdot 
x^{-\delta_{n-1} \Phi_{n-1}}
T^{[0]} (x),
\end{align}
where $d_x \assign \arg x$,
$d_{\zeta_n} \assign \arg \zeta_n$.
\end{lem}

\begin{prf}
Denote
$\Tilde{H}^{[0]}(x,\zeta_n)=
\left(
\frac{\zeta_n}{x}
\right)^{\ad \delta_{n - 1}\Phi_{n - 1}} 
H^{[0]}(x,\zeta_n)$.
Suppose that the systems \eqref{xzetaSys} 
has a common solution in the form of
$F^{[0]} (x, \zeta_n) 
\zeta_n^{-\delta_{n - 1}\Phi_{n - 1}}
X(\zeta_n)$, 
then we have
\begin{align*}
\frac{\partial}{\partial \zeta_n}  
(\Tilde{H}^{[0]} X)
= \frac
{\partial 
\Tilde{H}^{[0]}}
{\partial \zeta_n} 
X + 
\Tilde{H}^{[0]}
\frac
{\partial X}
{\partial \zeta_n}
= A_2 \cdot
\Tilde{H}^{[0]} X, 
\end{align*}
which can be rewrite as
\begin{align}
\label{T2eqLem}
\frac{\partial X}{\partial \zeta_n} \cdot 
X^{- 1} 
& = 
(\Tilde{H}^{[0]})^{- 1} A_2 
\Tilde{H}^{[0]} - 
(\Tilde{H}^{[0]})^{- 1} 
\frac{\partial \Tilde{H}^{[0]}}
{\partial \zeta_n}.
% \\
% \frac{\partial T^{[0]}}{\partial x} \cdot 
% (T^{[0]})^{- 1} 
% & = 
% (F_d^{[n]})^{- 1} A_1 F_d^{[n]} - 
% (F_d^{[n]})^{- 1} 
% \frac
% {\partial F_d^{[n]}}
% {\partial x} . 
\end{align}
From \eqref{Lim:adH1} and \eqref{Lim:addH1}
in Lemma \ref{Lem:CatPic},
we can verify $X(\zeta_n)$
satisfied the system \eqref{Eq:T2}
by taking the limit $x\to 0$
in \eqref{T2eqLem}.
Therefore, 
the systems \eqref{xzetaSys} 
has a common solutions
$F_{d_x}(x,\zeta_n/x)$ and
$F^{[0]}(x,\zeta_n) \cdot 
\zeta_n^{-\delta_{n-1} \Phi_{n-1}}
T^{[n]}_{d_{\zeta_n}} (\zeta_n)$.

Next, we fix $x$ and 
take the limit $\zeta_n\to\infty$. 
Condition \eqref{Cond:NonDengStokesS} 
ensures that at this time, 
the Stokes sector of $F_{d_x}$ 
containing the ray $\arg x=d_x$ will not degenerate.
From \eqref{Lim:Hd}, \eqref{Lim:H1}
and \eqref{Lim:adYd}
in Lemma \ref{Lem:CatPic},
we locally uniformly have
the following asymptotic expansion
\begin{align*}
F_{d_x}(x,\zeta_n/x) \cdot
C_{d_x} (u,\delta_{n-1}\Phi_{n-1})
&\sim
(I+o(1;\zeta_n))
\zeta_n^{\delta_{n-1}\Phi_{n-1}}
\mathe^{
\frac{\partial u_n}{\partial z_n}
\zeta_n E_n}\cdot 
x^{-\delta_{n-1} \Phi_{n-1}}
T^{[0]} (x),\\
F^{[0]}(x,\zeta_n) \cdot 
\zeta_n^{-\delta_{n-1} \Phi_{n-1}}
T^{[n]}_{d_{\zeta_n}} (\zeta_n)
&\sim
(I+o(1;\zeta_n))
\zeta_n^{\delta_{n-1}\Phi_{n-1}}
\mathe^{
\frac{\partial u_n}{\partial z_n}
\zeta_n E_n}\cdot 
x^{-\delta_{n-1} \Phi_{n-1}}
T^{[0]} (x),
\end{align*}
since the solution of the linear system 
is uniquely determined by 
its asymptotic leading term, 
we have
\begin{align*}
F_{d_x}(x,\zeta_n/x) \cdot
C_{d_x} (u,\delta_{n-1}\Phi_{n-1})
&=
F_{d_{\zeta_n}}^{[n]}(x,\zeta_n) \cdot 
x^{-\delta_{n-1} \Phi_{n-1}}
T^{[0]} (x),\\
F^{[0]}(x,\zeta_n) \cdot 
\zeta_n^{-\delta_{n-1} \Phi_{n-1}}
T^{[n]}_{d_{\zeta_n}} (\zeta_n)
&=
F_{d_{\zeta_n}}^{[n]}(x,\zeta_n) \cdot 
x^{-\delta_{n-1} \Phi_{n-1}}
T^{[0]} (x),
\end{align*}
thus we complete the proof.
\end{prf}\\

\begin{rmk}
\label{Rmk:PreCat}
Condition \eqref{Cond:NonDengStokesS} can
be rewritten as
\begin{align*}
u_n &\notin
\tmop{conv}\{u_1,\ldots,u_{n-1}\},\\
d_x &\notin
-\arg(u_n -
\tmop{conv}\{u_1,\ldots,u_{n-1}\})+
\mathbb{Z}\pi.
\end{align*}
It can be seen in \eqref{PreCat} that 
both sides of the identity should depend on 
both $\arg \zeta_n = d_{\zeta_n}$ 
and $\arg x = d_{x}$
at the same time, 
but the identity itself does not explicitly show it.
In fact
\begin{itemize}

\item When we fix $x$ and
$\zeta_n$ is large enough,
if $d_{\zeta_n}+
\arg(\frac{\partial u_n}{\partial z_n})=
\arg(\frac{\partial u_n}{\partial z_n}\zeta_n)$ 
crossed $\mathbb{Z}\pi$,
the Stokes sector of $F_{d_x}(x,\zeta_n/x)$
which contains the ray $\arg x=d_x$ 
on the left-hand side will change,
therefore the $F_{d_x}$ 
will not remain the same,
and the right-hand side
will naturally change in these crossing 
by the definition;

\item When we fix $\zeta_n$, 
the right-hand side
does not depend on the choice of $d_x$.
But under the condition \eqref{Cond:NonDengStokesS}, 
both $F_{d_x}$ and $C_{d_x}$ 
in the left-hand side 
will simultaneously change 
with the choice of $d_x$.
\end{itemize}
\end{rmk}


% \subsection{Proof of the Caterpillar Formula}

\begin{cor}
\label{Cor:PhikCat}
Suppose that $\Phi_{k-1}\in
\mathfrak{b}_{k-1}(\mathrm{pt})$ and
$\Phi_k=\mathcal{s}_k(\Phi_{k-1})$, then
\begin{align}
\label{CdDeng}
\lim_{z_k\to\infty}
C_{d}(u,\delta_k\Phi_k(z_k))
z_k^{-\delta_{k-1}\Phi_{k-1}}
z_k^{\delta_{k}\Phi_{k-1}}
& =
C_{d}(u,\delta_{k-1}\Phi_{k-1})
C_{d+\arg z_k}\left(
\frac{\partial u_k}{\partial z_k}E_k,
\delta_k\Phi_{k-1}\right),
\end{align}
where the argument of $z_k$ is 
restricted in a sufficiently small range.
\end{cor}

\begin{prf}
Since $\delta_k\Phi_k(z_k)$ 
satisfies the $k$-th isomondromy equation
with respect to $z_k$,
we can assume that $k=n$
without loss of generality.
Denote $z_n = \zeta_n/x$,
from \eqref{Lim:adH} and \eqref{Lim:adH1}
we have
\begin{align*}
  z_n^{\delta_{n - 1} \Phi_{n - 1}} F (x, \zeta_n / x) z_n^{- \delta_{n - 1}
  \Phi_{n - 1}} z_n^{\Phi_n} 
  & \xrightarrow{x \rightarrow 0} 
  T^{[n]}(\zeta_n),\\
  z_n^{\delta_{n - 1} \Phi_{n - 1}} F^{[0]} (x, \zeta_n) \zeta_n^{- \delta_{n
  - 1} \Phi_{n - 1}} T^{[n]} (\zeta_n) 
  & \xrightarrow{x \rightarrow 0}
  T^{[n]}(\zeta_n),
\end{align*}
By applying \eqref{PreCat} in Lemma \ref{Lem:PreCat},
we can complete the proof.
\end{prf}

\begin{lem}
\label{Lem:CatPsi}
Suppose that $\Phi_n(z)$ is 
the general solution of 
the $n$-th isomonodromy equation \eqref{zisoeq}
with boundary value $\Phi_0$,
and $z_1,\ldots,z_n$ are large enough,
then we have
\begin{align*}
\nu_{u,d}(\Phi_n(z)) & =
\tmop{Ad}\left(
\overrightarrow{\prod^n_{k=1}}
C_{d+\arg (u_k-u_{k-1}) }\left(
E_k
,\delta_k\Phi_0\right)
\right)
\mathe^{2\pi\mathi\Phi_0}.
\end{align*}

\begin{prf}
Denote $\Psi_k =
(z_k\cdots z_1)^{\ad\delta_k\Phi_k}
\Phi_k$, 
note that $\delta_k\Psi_k =
\delta_k\Phi_k$.
We inductively assume that
\begin{align}
\label{CatuRec}
\nu_{u,d}(\Phi_n(z)) & =
\tmop{Ad}\left(
C_{d}(u,\delta_k\Psi_k)
\overrightarrow{\prod^n_{j=k+1}}
C_{d+\arg (u_j-u_{j-1})}\left(
E_j
,\delta_j\Psi_k\right)
\right)
\mathe^{2\pi\mathi\Psi_k}.
\end{align}
rewrite \eqref{CdDeng} in Corollary \ref{Cor:PhikCat} as
\begin{align*}
\lim_{u_k\to\infty}
C_{d}(u,\delta_k\Psi_k)
u_k^{-\delta_{k-1}\Psi_{k-1}}
u_k^{\delta_{k}\Psi_{k-1}}
& =
C_{d}(u,\delta_{k-1}\Psi_{k-1})
C_{d+\arg (u_k-u_{k-1}) }\left(
E_k,
\delta_k\Psi_{k-1}\right),
\end{align*}
Therefore
\eqref{CatuRec} holds for $k+1$. 
Since
the induction starting point $k=n$
holds by definition, 
thus \eqref{CatuRec} inductively holds for $k=0$.
Note that $\Psi_0=\Phi_0$, 
we have completed the proof.
\end{prf}

\end{lem}



% \input{Thm/Thm_GenCat}
